Formation of primordial black hole binaries and their merger rates

We review the theory behind the formation of primordial black hole binaries and their merger rates. We consider the binary formation in the early and late Universe, emphasising the former as it gives the dominant contribution of the present primordial black hole merger rate. The binaries formed in the early Universe are highly eccentric so their interactions with other primordial black holes can significantly increase their coalescence times and thereby suppress the merger rate. We discuss in detail how the suppression of the merger rate arising from such interactions can be estimated and how such interactions lead to the formation of another, much harder, binary population that contributes to the present merger rate if more than 10% of dark matter consists of primordial black holes with a relatively narrow mass distribution. When the primordial abundance is below 1%, encounters between primordial black holes are unlikely and their effect on the merger rate becomes negligible.

==> report.tex <==
The authors present an introductory derivation of the merger rate of primordial black hole binaries from the various channels proposed in the literature. The chapter is overall well-written and accessible. Some parts of the derivation are more technical, but this is in line with the focus of the chapter. The detailed descriptions of the computations help follow and eventually reproduce the results.

I have the following suggestions to improve the presentation:

- In the abstract, it is stated that the early universe channel provides the dominant merger rate. However, in the following line, they state binaries get easily disrupted by interactions with other PBHs. While disruption is probably meant as "change in the binary parameters", it could be interpreted as the binary being broken into unbounded PBHs. I would suggest the authors rephrase this summary to improve clarity. I would also suggest stressing in the abstract that these encounters are unlikely if the abundance of PBH is small.
Also, it would be useful to define how "disruption" is used in the main text after its first appearance.

** We removed "disrupted" from the abstract and clarified this term in the main text in footnote 2. We included a sentence in the abstract specifying that encounters are less likely for small PBH abundances.

- 17.1.1: point 2. Define a "hard" binary. It would be useful to estimate whether initial PBH binaries are hard in typical environments expected in both the early or late universe.

** We define a hard binary in footnote 1. We included an estimate of hardness on page 19.

- 17.1.1 "Although this channel could also produce ABH-PBH binaries, their contribution is expected to be marginal." Can the authors describe why this is so? Is the low rate due to the small number density of both ABH and PBH in the environment where the two coexist?

** We have added a reference for this sentence.

- Footnote 5: Can the choice delta^2 = 0.005 be justified? Does different values of density perturbations have a large impact on the rates?

** We now discuss the effect of the size of matter perturbation below eq (17.43).

- "As the disruption of PBH binaries in late CDM haloes is very unlikely" below (17.41). It would be useful to explain in a few words the motivation supporting this statement. 

** We extended the discussion and added a reference to section 17.2.2.

- Eq. (17.53). What is the quantitative effect of subhaloes? Binary interactions are expected to be more frequent in smaller environments due to smaller velocities. Do sub-haloes have a dominant role? What are the uncertainties associated with the description of their mass function?

** We added curves showing the suppression factor neglecting the subhalo term in Fig. 6 and a comment that it becomes dominant around $f_{\rm PBH} = \mathcal{O}(0.1)$. Our estimate assumes that the subhalo mass function has a similar N dependence to the halo mass function. The velocity dependence is accounted for when computing the binary disruption probability within a subhalo. There is presently no estimate of the uncertainty of this suppression mechanism in the literature.

- Before eq. 17.42 the suppression SL is still not discussed. I would propose to move the summary of the merger rate formula after eq. (17.58).

** The suppression factor is discussed in eq (17.13).

- After eq. (17.79). Hardening may induce faster binary evolution and larger merger rates. It would be helpful to discuss why this effect is small compared to GW evolution and whether this result depends on PBH clustering.

** We added a sentence discussing this.

- Eq. (17.83) is unclear. The sum over different environments depends on N through the number density nN. However, also the rate  R1 can depend on N, in general, as in smaller virialized environments the velocities are smaller, thus increasing rates. This is mentioned later, but I would suggest the authors to explain this more carefully and potentially report the rate summed over N assuming virial velocities for clusters with N objects.

** We have fixed Eq. (17.83) by including the velocity dispersion.

- After (17.88):  "two-body capture process will quickly merge ". It would be interesting if the authors evaluated the merger timescale assuming the bmax impact parameter to show this explicitly.

** We have added the expression for the binary coalescence time as a function of the impact factor and shown that the coalescence time is very short.

- Fig. 17.8. Can the authors report a band around "late 3-body" varying gamma as they do for the early 3-body? 

** We have added the range as requested by the referee.

 - It would be interesting to report the upper bound from LVK on the merger rate of 30 Msun binary (no lower bound is found if no event is strictly assumed, or shown, to be primordial).

** We included a line indicating the LVK bound and a remark that the bound depends on the mass and time dependencies in the merger rate.

- It would also be very interesting to report a similar panel with the merger rates obtained for asteroidal mass/SMBH mergers, to show the variation of results as a function of the assumed mass. Both ranges are interesting per se, with the former being free from constraints on fPBH and of interest for ultra-high frequency GWs, while the latter is associated with the SMBH seed problem and LISA/PTA experiments. 

** We included another panel for 0.1 Msun to indicate how the merger rates scale with mass.

- The final comment on the effect of clustering is very interesting. Would it be possible to scale the suppression factors with a similar "fPBH-> delta fPBH" argument? I would give this comment more prominence, and stress a detailed description of the merger rate for clustered scenarios as well as very broad mass distributions is still lacking in the literature.

** The simple scaling holds for local effects, but not for processes affecting the binaries much after their formation. We have clarified this in the last paragraph of the chapter.

Minor points on the presentation:

- I would explicitly report the names used for subsections 17.2.1.1 - 17.2.1.3 in the list of effects described in the paragraph after (17.13). One could also include a reference to these sections. This would facilitate the reader, as these subsections are quite long and technical and a more explicit intro paragraph would help.

** We implemented the requested changes in the paragraph below (17.13).

The fourth point is discussed in 17.2.2. It should probably be 17.2.1.4 for consistency with the list above.

- Fig. 17.2 should appear on the next page, as it is only mentioned after eq. 17.23.

** We moved Fig. 17.2.

- fig. 17.6 is only mentioned on the following page. It should be moved below.

** Fig. 17.6 now appears on the same page as the reference to it.
